Light simulation in plastic scintillator strip with embedded wavelength shifting fiber

The simulation study of the light yield and attenuation in the plastic scintillator was performed. The wavelength shifting fiber readout was embedded in the grooves machined along the entire strip surface. The scintillator strips was irradiated with a radiation source {}^{90}Sr or cosmic muons along and across the strip.

==> texfig1a.tex <==
%%\begin{figure}[htbp]
\begin{figure}[ht!]                             %%   [H]      
{\hskip  1.0cm} \includegraphics[scale=0.65]{cos_muon.eps}
\caption[]{The azimutal angular distribution (left panel) and energy spectrum (right panel) of
cosmic muons as simulated according to\cite{volk}.} 
\label{Norm}
\end{figure}

